Canopy: Exploiting Piecewise Smooth Tree Priors for Multi-Fidelity Bandits

Many LLM inference problems, including model routing, prefix-cache management, prompt trimming, and test-time search, can be viewed as optimization over a tree. This structure arises naturally from autoregressive generation: every prefix defines a node, and its continuations form a subtree below it. Internal nodes of the tree provide cheap but biased estimates of a region's value, while leaf evaluations are expensive but accurate. Hierarchical bandit methods can exploit this structure, but typically require a specific smoothness schedule to be specified in advance, even though real objectives are often only piecewise smooth and their optima may lie near sharp boundaries. We introduce CANOPY, a multi-fidelity tree bandit that learns where the smoothness prior is valid rather than assuming it globally. CANOPY uses cheap random-path probes to construct an online certificate of local aggregation bias, then directs expensive leaf evaluations toward cells where the certificate detects a smoothness violation. We prove fixed-budget and regret guarantees whose additional cost is additive in the number of discontinuities, recovering the smooth-tree rate when no violations are present and approaching structure-blind search as violations become dense. Across routing, top-$k$ identification, test-time search, caching, and prompt trimming, CANOPY consistently improves matched-budget performance, including $2.9\times$ higher top-10 recall on a 1000-model pool, $1.6\times$ more SWE-bench Verified issues resolved than best-of-$N$, and $3.6\times$ lower median time-to-first-token with prefix caching.

==> figures/mmlu_routing_table.tex <==
\begin{tabular}{lrrr}
\toprule
Policy & Regret & Avg.\ quality & Rel.\ cost/query \\
\midrule
Hierarchical (ours) & 472 $\pm$ 3 & 0.977 $\pm$ 0.001 & 0.254 $\pm$ 0.002 \\
Flat (structure-blind) & 878 $\pm$ 8 & 0.943 $\pm$ 0.001 & 0.363 $\pm$ 0.006 \\
Best single (oracle ref.) & 831 $\pm$ 8 & 0.936 $\pm$ 0.001 & 0.316 $\pm$ 0.000 \\
Highest-quality (oracle ref.) & 843 $\pm$ 4 & 0.969 $\pm$ 0.001 & 0.432 $\pm$ 0.000 \\
Per-prompt oracle & 0 $\pm$ 0 & 1.000 $\pm$ 0.000 & 0.067 $\pm$ 0.001 \\
\bottomrule
\end{tabular}


==> figures/reasoning_models_gpqa_diamond_table.tex <==
\begin{tabular}{lccc}
\toprule
Model & best-of-N [95\% CI] & value-guided [95\% CI] & $\Delta$ [95\% CI] \\
\midrule
\texttt{llama8b} & 0.258 [0.20, 0.32] & 0.263 [0.20, 0.32] & $+0.005$ [-0.07, +0.08] \\
\texttt{sonnet45} & 0.313 [0.25, 0.38] & 0.672 [0.61, 0.74] & $+0.359$ [+0.27, +0.44] \\
\texttt{llama3-1-70b} & 0.323 [0.26, 0.39] & 0.399 [0.33, 0.46] & $+0.076$ [+0.00, +0.15] \\
\texttt{nova-pro} & 0.354 [0.29, 0.42] & 0.414 [0.35, 0.48] & $+0.061$ [-0.01, +0.13] \\
\texttt{mistral-large} & 0.374 [0.31, 0.44] & 0.333 [0.27, 0.40] & $-0.040$ [-0.11, +0.04] \\
\bottomrule
\end{tabular}


==> figures/reasoning_models_gsm8k_table.tex <==
\begin{tabular}{lccc}
\toprule
Model & best-of-N [95\% CI] & value-guided [95\% CI] & $\Delta$ [95\% CI] \\
\midrule
\texttt{llama8b} & 0.925 [0.89, 0.96] & 0.850 [0.80, 0.90] & $-0.075$ [-0.12, -0.03] \\
\texttt{nova-pro} & 0.945 [0.91, 0.97] & 0.970 [0.94, 0.99] & $+0.025$ [+0.01, +0.05] \\
\texttt{mistral-large} & 0.955 [0.93, 0.98] & 0.840 [0.79, 0.89] & $-0.115$ [-0.16, -0.07] \\
\texttt{llama3-1-70b} & 0.960 [0.93, 0.98] & 0.960 [0.93, 0.98] & $+0.000$ [-0.03, +0.03] \\
\texttt{sonnet45} & 0.985 [0.96, 1.00] & 0.980 [0.96, 0.99] & $-0.005$ [-0.02, +0.00] \\
\bottomrule
\end{tabular}


==> figures/reasoning_models_math_table.tex <==
\begin{tabular}{lccc}
\toprule
Model & best-of-N [95\% CI] & value-guided [95\% CI] & $\Delta$ [95\% CI] \\
\midrule
\texttt{mistral-large} & 0.084 [0.05, 0.12] & 0.140 [0.10, 0.18] & $+0.057$ [+0.01, +0.10] \\
\texttt{sonnet45} & 0.503 [0.45, 0.56] & 0.837 [0.79, 0.88] & $+0.333$ [+0.28, +0.39] \\
\texttt{llama8b} & 0.537 [0.48, 0.59] & 0.390 [0.34, 0.45] & $-0.147$ [-0.21, -0.09] \\
\texttt{llama3-1-70b} & 0.540 [0.48, 0.59] & 0.607 [0.55, 0.66] & $+0.067$ [+0.02, +0.12] \\
\texttt{nova-pro} & 0.623 [0.57, 0.68] & 0.753 [0.70, 0.80] & $+0.130$ [+0.08, +0.18] \\
\bottomrule
\end{tabular}


==> figures/swebench_sweep_table.tex <==
\begin{tabular}{lccc}
\toprule
Model & $B=6$ & $B=9$ & $B=12$ \\
\midrule
claude-sonnet-4.5 & \textbf{$+0.100$ [+0.02, +0.19]} & \textbf{$+0.125$ [+0.04, +0.21]} & $+0.062$ [-0.01, +0.14] \\
nova-pro & \textbf{$+0.100$ [+0.03, +0.18]} & $+0.062$ [-0.01, +0.15] & $+0.025$ [-0.04, +0.09] \\
llama-3.1-70B & $+0.050$ [-0.01, +0.12] & \textbf{$+0.087$ [+0.02, +0.16]} & $+0.025$ [-0.04, +0.09] \\
mistral-large & $+0.013$ [-0.04, +0.06] & $+0.013$ [-0.04, +0.06] & $-0.013$ [-0.06, +0.04] \\
llama-3.1-8B & $-0.013$ [-0.08, +0.05] & $+0.050$ [+0.00, +0.11] & $+0.037$ [-0.02, +0.10] \\
\bottomrule
\end{tabular}


==> figures/taubench_replicates_table.tex <==
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{2}{c}{regional (ours)} & \multicolumn{2}{c}{flat} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
Replicate & success & \$/task & success & \$/task \\
\midrule
1 & 0.450 & 0.0478 & 0.100 & 0.0078 \\
2 & 0.537 & 0.0620 & 0.225 & 0.0141 \\
3 & 0.225 & 0.0173 & 0.537 & 0.0672 \\
4 & 0.450 & 0.0367 & 0.188 & 0.0168 \\
5 & 0.650 & 0.0613 & 0.562 & 0.0703 \\
\midrule
mean $\pm$ s.d. & 0.463 $\pm$ 0.156 & & 0.323 $\pm$ 0.213 & \\
\bottomrule
\end{tabular}


==> figures/taubench_routing_table.tex <==
\begin{tabular}{lrr}
\toprule
Policy & Task success [95\% CI] & Avg.\ cost/task (\$) \\
\midrule
\textbf{routed-flat} & \textbf{0.100 [0.04, 0.17]} & \textbf{0.00778} \\
\textbf{routed-regional (ours)} & \textbf{0.450 [0.34, 0.56]} & \textbf{0.04781} \\
nova-micro-v1 & 0.125 [0.05, 0.20] & 0.00226 \\
nova-lite-v1 & 0.150 [0.07, 0.24] & 0.00533 \\
llama3-1-8b-instruct-v1 & 0.138 [0.07, 0.21] & 0.01897 \\
llama3-1-70b-instruct-v1 & 0.150 [0.07, 0.24] & 0.05993 \\
claude-sonnet-4-5-20250929-v1 & 0.600 [0.49, 0.70] & 0.07820 \\
mistral-large-2402-v1 & 0.163 [0.09, 0.25] & 0.08188 \\
\bottomrule
\end{tabular}

